Learning to Structure Long-term Dependence for Sequential Recommendation

Sequential recommendation recommends items based on sequences of users' historical actions. The key challenge in it is how to effectively model the influence from distant actions to the action to be predicted, i.e., recognizing the long-term dependence structure; and it remains an underexplored problem. To better model the long-term dependence structure, we propose a GatedLongRec solution in this work. To account for the long-term dependence, GatedLongRec extracts distant actions of top-$k$ related categories to the user's ongoing intent with a top-$k$ gating network, and utilizes a long-term encoder to encode the transition patterns among these identified actions. As user intent is not directly observable, we take advantage of available side-information about the actions, i.e., the category of their associated items, to infer the intents. End-to-end training is performed to estimate the intent representation and predict the next action for sequential recommendation. Extensive experiments on two large datasets show that the proposed solution can recognize the structure of long-term dependence, thus greatly improving the sequential recommendation.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)

==> outline.tex <==
\textbf{sequential pattern can indicate users' interest}
Driven by evolving interest, users interact with items sequentially on online service platforms like e-commerce website or news media website. The sequential order of actions leaks the dynamics of users' interest. To understand the dynamics of users' interest and then satisfy users' dynamic need, sequential recommendation models actions in sequential fashion as how they are generated by users and leverages the sequential transition patterns among actions. Specifically, sequential recommender is to predict the item of the next action (target action) that a user would interact with based on a sequence of actions generated by this user, and to recommend the user a list of items which are the most relevant to the user's interest.

\textbf{sequential recommendation is to leverage sequential pattern for recommendation}

\textbf{what is the challenge?}

Sequential recommendation is given a sequence of a certain user's actions in chronological order, to predict the item of the next action (target action), and then recommend a list of the most relevant predicted items to the user. Leveraging sequential pattern among actions via treating actions as sequences enables sequential recommender to understand the dynamics of users, thus providing relevant items to meet users' evolving interest and improving the recommendation quality.

Q: Why sequential recommendation?
A: Sequential patterns that the items which a certain user has historically interacted with may indicate the next item which the user would choose 

Users sequentially interact with the system. The items which a certain user has historically interacted with may indicate the next item which the user would choose. Sequential patterns have been leveraged by sequential recommender to improve the recommendation quality.

Q: what is sequential recommendation? 
A: Sequential recommendation is given a sequence of a certain user's actions in chronological order, to predict the item of next action, and then recommend a list of the most relevant predicted items to the user. 

User sequentially interact with the system sequentially. The sequential pattern, i.e. the items which a certain user has historically interacted with can indicate the next item which the user would choose, has been leveraged by sequential recommender to improve the recommendation quality. Sequential recommendation is given a sequence of a certain user's historical actions in chronological order, to predict the item of the next action (target action), and then recommend a list of the most relevant predicted items to the user. It has been verified that not only recent actions (within $M$ steps range to the target action) can indicate the target action, but also long-range actions (more than $M$ steps range to the target action) can indicate the target action. Take as an example the sequence of actions generated by a certain user in online shopping website shown in Figure~\ref{fig:Sequence_example_intro}. Both recent clicks and long-range clicks can indicate the items that the user would click in target actions. 


It has been verified that not only recent actions can indicate the target action, but also long-range actions can indicate the target action.


JW) The above two questions could be brief in one or two sentence
try to emphasize the idea of range in the definition and use case of sequential recommendation, so it is natural to move forward on the challenge about modeling long range

Q: Why long-term dependence in sequential recommendation? 
A: xxx work show that the sequential pattern does not only exist among recent actions but also exist among long-range actions, but they are heterogeneous \textbf{need more explanation about what the difference is?}. xxx work show that short-term dependence is useful to sequential recommendation and xxx work show that long-term dependence is also beneficial to sequential recommendation. But most work on leveraging sequential pattern for sequential recommendation focus on short-term dependence, while long-term dependence gets little attention. From applying Markov Model to Neural Models, these methods are designed to capture short-term dependence. 

Q: what the challenge of modeling long-term dependence in sequential recommendation?
A: As the number of actions separating the target action and a certain long-range action is large and the action space is huge, the structure of the dependence carried on these actions can be quite complex. 


A: First, the long-term dependence is high-order. As the target action and a certain long-range action are separated by a few other actions, the dependence on this certain long-range action may be correlated with other actions in between. Consequently, the order of dependence is correlated with the number of actions in between, which is generally high. Second, the long-term dependence is context dependent. Generating actions of different items may be influenced by different sub-sequences of actions. For example, the action of clicking a bag may be influenced by actions of clicking bags.  


Why long-term dependence? 

There exist two types of dependence but they are different. 

As previous work shows, the sequential transition pattern exist not only among contiguous actions, but also among distantly separated actions. Therefore, to predict the user's interest for target action, the sequential recommender should consider the dependence of target action on both recent actions which are within several steps to the target action and long-range actions which are far apart from the target action. On the other hand, due to the different sequential steps towards the target action, the dependence on recent actions is different from that on long-range actions~\cite{}. Due to the small distance, the interest underlying recent actions would be similar to that driving the target action. In contrast, because of the long distance the interest underlying long-range actions would diversify. Some could be driven by totally different interest while some could be driven by closely related interest. Therefore, differentiating these two types of dependence is necessary for sequential recommender.  

Take as an example the sequence of actions generated by a user on online shopping website, which is shown in Figure~\ref{fig:Sequence_example_intro}. Because of close distance, recent browsing including bags and cloths may influence the choice of the bag of the target action ``A". While, due to large distance, long-range actions of browsing bags may still affect the choice for target action ``A". 

The bag browsed in the target action  may be influenced both by recent actions of browsing bag and long-range actions of browsing bags. 

Unfortunately, most work on leveraging sequential pattern for sequential recommendation focus on modeling the dependence of target action on recent actions. From Markov Chain based models to RNN based models, they are designed to capture the dependence on actions in a short-range. When applying to capture the transition pattern among far apart actions in long sequences, Markov Chain based models suffer from the exponentially growing state-space. Due to the gradient diminishing issue, RNN does not perform well on modeling long sequences. So far, the dependence on long-range actions are undermined to improve the recommendation quality. One major challenge is the complex structure of the dependence on long-range actions. As long-range actions are tens or hundreds steps apart from the target action and the action space is huge, the interest driving long-range actions are subtly coupled with the interest driving target action. Among actions driven by diverse interest, differentiating actions which may closely related to target action from irrelevant actions becomes difficult.

Recently, enhancing the capture of the dependence on long-range actions attracts researchers' attention. \citet{quadrana2017personalizing} proposed a hierarchical RNN where a RNN captures the dependence among actions within-session and the other RNN captures dependence among actions across sessions by taking the output of within-session RNN as input. This method treats past actions within a session as recent actions and treats actions across sessions as long-range actions. Assuming that the dependence on long-range actions are built with hierarchical structure, this method organizes long-range actions into binary tree where a node represents a session of actions. The level of the node in the tree is determined by the order of the corresponding session in the sequence. Likewise, \citet{you2019hierarchical} also assumed the dependence on long-range actions is developed with hierarchical structure and proposed a hierarchical model which replaces within-session RNN with TCN for the sake of the training speed. Reducing the path between long-range action and the target action allows these methods to capture the dependence among long-range actions, which has been shown to be helpful to improve the recommendation quality. Although the hierarchical structure is critical to the success of their methods, it also limits these methods' performance. With the hierarchical structure, all actions are assumed to have influence on the target action. These methods do not differentiate actions driven by closely related interest from actions driven by irrelevant interest. As a result, the sequential transition pattern recognized by these models become blur and inaccurate.

In this paper, we propose a neural sequential recommender which enhances the capture of the dependence on long-range actions in the meanwhile captures short-term dependence. As the structure of items organized with respect to items' categories can indicate the structure of users' interest~\cite{zhu2018learning}, we assume the actions of the same category (which means the items associated with the actions belong to the same category) are driven by closely related interest. To differentiate the dependence on long-range actions driven by closely related interest from the dependence on ones driven by irrelevant interest, we assume the target action depends on long-range actions of the same category while independent to other long-range actions. In this way, the dependence on long-range actions is contextualized towards the target action. Because the category of the target action to predict is unknown, we employ a gating network to predict the category of the target action. As recent actions can provide signals for users' interest, the gating network takes recent actions as input. Incorporating these components, our model employs a short-term encoder to capture the dependence on recent actions, a gating network to control which sub-sequences of long-range actions should be considered for the dependence of the target action, and a long-term encoder to capture the dependence on selected long-range actions. To leverage different sequential patterns buried in recent actions and long-range actions, we use a RNN as short-term encoder and the other RNN as long-term encoder. We fuse the dependence captured by short-term encoder and the dependence captured by long-term encoder to represent the user' interest for the target action. With respect to the user' interest, we compute items' relevance and recommend a list of the most relevant items to the user. We name our model as GateLongRec.

% As the root node of a sub-tree in the hierarchical structure blocks the dependence passing from the leaf node of the sub-tree to other nodes in the tree, the dependence on long-range actions of the sub-tree are independent towards target action. As a result, no matter 

In this work, we propose a sequential neural recommender to capture the dependence among actions accurately, which especially can capture the dependence on long-range actions accurately. As previous work suggest that the property of the dependence on recent actions is different from that of the dependence on long-range action~\cite{tang2019towards, quadrana2017personalizing}, our model decomposes the dependence on historical actions into the dependence on recent actions (short-term dependence) and the dependence on long-range actions (long-term dependence). To enable the long-term dependence adaptive towards the target action, our model employs a gating network controlling which sub-sequence of actions should be considered for long-term dependence, and the gating network is correlated with the target action. As categories can indicate users' interest and the category information is widely available in many domains~\cite{zhu2018learning}, we believe it is reasonable to assume that the category information of the target action can serve as signal indicating which sub-sequence of actions have influence on the target action. Therefore, the gating network is to predict the category of the target action. In this way, the target action depends on long-range actions of the same category predicted by the gating network. On the other hand, we employ a RNN over recent actions to account for the short-term dependence. To predict the item of the target action, we fuse short-term dependence and long-term dependence. For recommendation, we rank items according to their prediction score in descending order and select a list of top ranked items. We jointly optimize the task of predicting the item of the target action and the task of predicting the category of the target action. We name our model as GateLongRec.

% As the hierarchical structure developed by these methods is binary tree, the dependence on long-range actions which are in the bottom level of the tree is fixed and independent from the target action. In addition, the hierarchical structure is fixed 

% Because of the hierarchical structure, the distance between long-range actions and the target action reduces, which mitigates the gradient dimin

% The high-level RNN takes the low-level RNN's output as input and the output of high-level RNN represents the influence of long-range actions. Likewise, \citet{you2019hierarchical} proposed a hierarchical model combining RNN with TCN to speed up the recommendation. As these models segment a sequence into chunks and then employ RNN over these chunks, the gradient diminishing issue resulting from long sequences is mitigated. Through hierarchical structure, these models can take in account the influence of long-range actions. 


% As the number of actions separating the target action and a certain long-range action is large and the action space is huge, the structure of the dependence carried on these actions can be quite complex. 

 


